End-to-end Tracking with a Multi-query Transformer

Multiple-object tracking (MOT) is a challenging task that requires simultaneous reasoning about location, appearance, and identity of the objects in the scene over time. Our aim in this paper is to move beyond tracking-by-detection approaches, that perform well on datasets where the object classes are known, to class-agnostic tracking that performs well also for unknown object classes.To this end, we make the following three contributions: first, we introduce {\em semantic detector queries} that enable an object to be localized by specifying its approximate position, or its appearance, or both; second, we use these queries within an auto-regressive framework for tracking, and propose a multi-query tracking transformer (\textit{MQT}) model for simultaneous tracking and appearance-based re-identification (reID) based on the transformer architecture with deformable attention. This formulation allows the tracker to operate in a class-agnostic manner, and the model can be trained end-to-end; finally, we demonstrate that \textit{MQT} performs competitively on standard MOT benchmarks, outperforms all baselines on generalised-MOT, and generalises well to a much harder tracking problems such as tracking any object on the TAO dataset.

==> sections/model.tex <==
\section{dDETRactor}
The backbone of our model is a deformable DETR (dDETR)~\cite{zhu2021ddetr} detection transformer. For the purpose of tracking, we leave the encoder module of the transformer largely untouched and solely focus on the decoder module. In the traditional decoder, the set of output embeddings is initialized with so-called query embeddings. 

\subsection{Tracking mechanism}
\noindent\textbf{Track initialization:} In the problem of tracking, for a video sequence we are given the initial location of the object. We can either leverage this information by encoding each track according to its position using the provided location, or we can initialize the objects from a static query. We find that the former is preferable if the annotations are accurate, but the latter allows us to detect new objects in the frame if annotations are not reliable. Note that for the evaluation on MOT17~\cite{MOT16and17} tracking works refer to the \textit{private and public detections}. \textit{Public} detections are provided with the dataset and allow for a comparison of tracking methods independent of the object detection performance of the model. \textit{Private} detection setting during evaluation allows for the use of the available object detector for track initialization. For our evaluation, if the setting is marked as \textit{public}, we initialize the model with dataset detections; if marked \textit{private}, we initialize the tracks with static \texttt{rand} queries. If marked as \textit{private + public}, we use both and rely on the set-matching algorithm to find an optimal mapping to the ground-truth tracks. 


\noindent\textbf{Tracking:} For each query at \textit{i}-th step, we generate a corresponding output embedding $V^i_{|k}$ where $k$ denotes query type, and two downstream embeddings $b^i_{|k}$ and $a^i_{|k}$ encoding location (bounding box) and location respectively. These then became queries semantic queries for the known tracks that are auto-regressively sent to the decoder for the next step. At each subsequent step, we feed these three outputs to the decoder, each of them producing three of their own output embeddings that are then aggregated in order to produce the new location and appearance vectors. Outputs are at each step matched to the ground truth, and for each lost track a reID is attempted from the \texttt{rand} queries at each tracking step. The tracking scheme is loosely illustrated in Figure~\ref{fig:splash}, and more details are given in Figure~\ref{fig:2stagetraining}. The exact architecture is discussed in more detail in the supplementary material. 



\subsection{Semantic queries: track confirmation and reID}
Given that dDETRactor produces high-level features for each track and is able to \textit{attend} over multiple objects in the frame (thus being able to reason about their locations and appearances), we argue that an entire network for reID of the tracks is not necessary. To this end, we show several simplified reID schemes that match or surpass the performance of~\cite{bergmann2019bells}. We ablate the methods in Table~\ref{abl:reid}.

\noindent\textbf{Direct similarity: }
The simplest, and yet effective tracking policy is to directly compare the cosine similarity between the embeddings for pairwise objects. Let $V^\cdot_{| \cdot)}$ represent the decoder embedding of an image given the query. Then we can say that the $p$-th embedding of the $i$-th frame matches $q$-th embedding of the $i+j$-th frame if $q$ is the embedding with minimum cosine distance and cosine distance between $V^i_{| b_{i-1}^p}$ and $V^i_{| b_{i-1}^q}$ is smaller than hyper-parameter $\tau_{\text{cos}}$. The two tracks match if the following conditions are met:

\begin{eqnarray}
\begin{cases} 
\begin{array}{rl}
q &= argmin_j( d(V^i_{| b_{i-1}^p)}, V^{i+1}_{ | b_i^j}) ) \\
\tau_{\text{cos}} & > d(V^i_{| b_{i-1}^p)}, V^{i+1}_{ |b_{i}^q}))
\end{array}
\end{cases}
\end{eqnarray}
where $d(\cdot, \cdot)$ is cosine distance between two embeddings. Note that there is no incentive for the model to produce embeddings that would be close to one-another in the latent space. 

\noindent\textbf{Learned similarity: } Thus, we decide to train an additional head over bare decoder embedding (we denote each head with a subscript, eg. $\phi_{\text{app}}$ for the appearance head).  We can train this embedding of $p$-th query to be similar to the embedding for a corresponding query several frames apart, and dissimilar to the embeddings produced by the decoder for all other queries in that frame.

\noindent\textbf{Additional semantic queries: } \citet{yu2021relationtrack} however, show the benefits of disentangled representations for tasks of detection and reID. Instead of using a joint embedding $V$ a single query for each object, we feed multiple queries per object to the decoder, each initialized in a different way, to produce multiple outputs for each object in the frame. More specifically, the decoder input queries as step $k$ are initialized from decoder \textit{output} embeddings from the step $k-1$. For each object, we will have queries corresponding to the: 1) predicted bounding box ($b$), 2) predicted appearance vector ($a$) and 3) output decoder embedding containing information about both location and appearance ($V$). If a set of queries is corresponding to a known track, a learned "tag" embedding (akin to positional embeddings) is added to them in order for the detector to know that they refer to the same object). Outputs of corresponding embeddings can then be aggregated via either average- or max-pooling, or an aggregation scheme such as the collaborative-gating~\cite{liu2019use}.

\subsection{Training the tracker:} \label{sec:training_deets}
In order to be able to track objects frame-to-frame, we train the DETRactor on two adjacent frames as indicated in Figure~\ref{fig:2stagetraining}. At the initialization step, we compute object detection loss from either input bounding-boxes via semantic queries or static random queries. In the tracking step, we optimize the model jointly for location prediction and appearance matching (i.e.\ tracking) for all non-background class objects initialized in the initialization step. 
The mapping from the ground truth objects in a given frame and the set of predictions from our model is determined via track identity or via costs based on the bounding-box similarity, class, and (if available) appearance. In the first case, tracks from the init step are matched to the output of the tracking step based on the cosine similarity of their output appearance vectors. If the track is "lost", i.e. the appearance vector at the current step doesn't match the appearance vector of the corresponding query at the init step (e.g.\ due to occlusions or objects moving out of the scene), we follow~\cite{carion2020DETR} and try to find injective minimum cost mapping between the ground truth and the set of predictions generated by static (\text{rand}) queries.

\noindent\textbf{Pseudo-tracking datasets: } Training the large transformer models requires a lot of training data, therefore we follow~\cite{trackformer} and simulate tracking data from COCO (in order to run ablations on object detection) and Crowd-Human~\cite{shao2018crowdhuman}. As in~\cite{trackformer}, the adjacent frames are generated by applying random spatial augmentations of up to 5\% with respect to the original image size. For COCO, we apply an additional constraint that no objects should be lost between the transformations. 

